Modeling and Analysis of Converged Network-Cloud Services

Networks connecting distributed cloud services through multiple data centers are called cloud networks. These types of networks play a crucial role in cloud computing and a holistic performance evaluation is essential before planning a converged network-cloud environment. We analyze a specific case where some resources can be centralized in one datacenter or distributed among multiple data centers. The economy of scale in centralizing resources in a sin- gle pool of resources can be overcome by an increase in communication costs. We propose an analytical model to evaluate tradeoffs in terms of application requirements, usage patterns, number of resources and communication costs. We numerically evaluate the proposed model in a case study inspired by the oil and gas industry, indicating how to cope with the tradeoff between statisti- cal multiplexing advantages of centralization and the corresponding increase in communication infrastructure costs.

==> Intro_submitted_SBRC.tex <==
\section{Introduction}
\label{sec:Intro}


Cloud computing is a large-scale distributed computing paradigm that is
driven by economies of scale, in which a pool of computing resources (e.g., networks, servers, storage, applications, and services) 
are provisioned, delivered and released on demand to users over a network \cite{foster2008cloud}. 
To the user, the available capabilities often appear to be unlimited and can
be elastically provisioned in any quantity at any time \cite{mell2011nist}. 

To improve cloud performance and resiliency, the current trend is to deploy the services across multiple and geographically distant sites
\cite{CloudNetworks}.
In this context, cloud networks (networks connecting cloud services hosted in multiple datacenter) play a crucial role in cloud computing 
and are an indispensable ingredient
for high performance cloud computing \cite{duan2012survey}.


In this paper we analyse a federated network cloud composed by multiple private or public clouds
hosting a software floating licensing cloud service. 
Floating licensing is a software licensing approach in which a limited number of licenses for an application is shared among a larger 
number of users over time and is often used for high-value applications in corporate environments \cite{hamadani1998automatic}.
The licenses are stored in a pool of licenses.
When a user wishes to run the application, a license is requested to a license server.
The task of a software license server is to determine and control the permitted number of copies of a software program based on the 
license entitlements that an organization owns. If a license is available, the license server allows the application to run. 
When the user finishes the application, the license is reclaimed by the license server 
and made available to other users. To avoid user's misbehaviour, the application periodically sends license renewal requests to the license server.
If the client does not receive an answer, a timeout is detected and the application is closed.

The federated clouds are linked by network cloud in such a way that backgroud traffic originated by others applications hosted in the cloud 
compete with the request/response licensing traffic. All the licenses can be consolidated in a single pool (Figure \ref{CentralizedLicenseServers})
or distributed in multiple pools (Figure \ref{RemoteLicenseServers}). 
The single pool explores the
statistical multiplexing gains due to resource sharing. Nonetheless, such economy of scale gains might 
overcome by an increase in communication costs, due to congestion generated by competing traffic from other applications in the cloud.
\emph{How to quantify and advantages and disadvantages of consolidating resources in a single pool?}

While partially answering the question above, our key contributions are the following:

\begin{enumerate}
\item \textbf{analytical model: } We propose an analytical model to capture the tradeoffs involved in resource centralization between  
gains due to statistical multiplexing and costs due to congestion;
\item \textbf{license serving analysis: } We apply our model to the analysis of how to distribute licenses in a cloud environment.  
To the best of our knowledge, this work is the first to study the license serving problem in a systematic way;
\item \textbf{case study: } we numerically investigate the proposed model using an case inspired by a real-world oil and gas setup.
\end{enumerate}


The remainder of this paper is organized as follows: Related work are discussed in Section \ref{sec:trabalhos_relacionados}.
In Section \ref{sec:modelo} we present the proposed analytical model. 
Section \ref{sec:exemplos} contains the numerical examples and Section \ref{sec:conclusions} concludes the paper.

\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.99\textwidth]{Centralized_Pool.jpg}
\end{center}
\caption{Centralized License Servers}
\label{CentralizedLicenseServers}
\end{figure}



\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.99\textwidth]{Distributed_Pool.jpg}
\end{center}
\caption{Remote License Servers}
\label{RemoteLicenseServers}
\end{figure}


==> modelo_licensing_reseting.tex <==
\section{Analytical Model}
\label{sec:modelo}

\subsection{Notation}

\begin{table}[h!]
\center
\begin{tabular}{ll}
variable & description \\
\hline
$N$ & number of pools \\
$S$ & population size \\
$S_i$ & population at pool $i$ \\
$L$ & number of licenses \\
$L_i$ & number of licenses at pool $i$ \\
\end{tabular}
\caption{Table of notation}
\end{table}

\begin{equation}
S=\sum^N_{i=1}S_i 
\end{equation}


\begin{equation}
L=\sum^N_{i=1}L_i 
\end{equation}

\subsection{One Centralized Pool of Licenses}



\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.6\textwidth, angle =270 ]{centralized_pool.eps}
\end{center}
\caption{Centralized License Servers}
\label{P_timeout}
\end{figure}

$\lambda$ =  request arrival rate

$1/\mu$ = average duration of a session, in minutes

$C$= circuit capacity

$\lambda_c$ = request arrival rate to circuit $C$

$1/\mu_c$ = average service in circuit $C$

$r$=rate at which licenses are checked (e.g., if $r=2$ it means that the license is checked 2 times per minute, while the session is active)

$W$ = random variable characterizing time for license expiration

$w=E(W)$=average license expiration time (mean time for license to expire, in minutes)

\begin{equation}
P(sucesso)=(1-P(bloqueio)) (1-P(timeout)) 
\end{equation}




\subsection{Blocking}


% \begin{equation}
% P(bloqueio)=\sum^{M}_{L+1} \binom{M}{L+1}p^{L+1}(1-p)^{M-(L+1)}
% \end{equation}


The blocking probability with finite sources is given by the \textit{Engset formula} \cite{teletraffic} 

\begin{equation}
P(blocking)=\frac{\binom{S-1}{L}(\frac{\lambda}{\mu})^L}{\sum^{L}_{i=0}\binom{S-1}{i}(\frac{\lambda}{\mu})^i}
\end{equation}


%\subsection{Timeout}

\subsection{Timeout due to congestion}

In this section we assume that each client periodically sends  license renewal requests 
to the license server, at a constant rate of  $r$ requests per second.
Each license renewal request is also referred to as a \emph{probe}.  
If the client doesn't receive an answer in $\tau$ seconds ($\tau < 1/r$), a timeout is detected 
and the application is closed. 
Note that due to network congestion, the chances of occurring a timeout if 
the license server is
centralized are higher than if the license server remains closer to end-users.



%In the centralized scenario, due to congestion, the waiting time in queue
% can be greater than $\tau$ seconds. The question addressed here
% is the probabilty of timeout due to congestion.}

Let $D_i$ be the duration of the $i$-th subinterval in which the license is checked.
Let $N$ be the number of times that probes are sent to the server until a timeout is 
generated, without counting the last probe ($N \ge 0$).
Let $q$ be the probability that a probe successfully yields a license renewal. Then,
   $N \sim Geometric(1-q)$, 
\begin{equation}
P(N=n)=q^n (1-q)
\end{equation}
Let $D$ be the time until a timeout, where $D$ is given as a function of $D_i$ and $N$ 
as follows,
\begin{equation}
  D = D_0 + D_1 + D_2 + \ldots + D_N  + D_{N+1} \\
  \label{D}  
  \end{equation}
  where $D_0=0$.   
In the remainder of this section we assume that 
$D_i\sim Constant(\frac{1}{r})$ for $i=1, 2, 3, \ldots$ but 
the argument presented below easily generalizes for the case where $D_i$ has general distribution, 
and  $D_1, D_2, \ldots$ are independent and identically distributed. The Laplace transform
of $D$ is given by
\begin{equation}
   D^{\star}(s) =  N(z)\bigg|_{z=e^{-(\frac{s}{r})}} D_{N+1}^{\star}(s) \\
  \label{D_star}
  \end{equation} 
where $N(z)$ is the z transform of $N$,
   \begin{eqnarray} \label{eqnz}
     N(z) &=&  \frac{1-q}{1- z q} 
  \end{eqnarray}
and
\begin{equation} \label{eqdi}
    D_{N+1}^{\star}(s) = D_i^{\star}(s) = e^{-s/r}, \qquad i=1, 2, 3, \ldots
\end{equation}
We substitute~\eqref{eqnz} and ~\eqref{eqdi}  into~\eqref{D_star} to obtain
\begin{eqnarray}
    D^{\star}(s) &=& e^{-{s}/{r}}\bigg( \frac{1-q  }{1- e^{-{s}/{r}}q }\bigg) 
%     D(k) &=& p^{k-\frac{1}{r}}(1-p)
\label{D_star_fim}
\end{eqnarray}

The \emph{target session duration}  is the desired duration of the session as determined
by the user requirements.   
Let the target session duration time be exponentially distributed with mean $1/\mu$,
 and let $L$ be the random variable that characterizes
the target session duration, $L \sim Exponential(\mu)$.  The actual session duration 
might be smaller than the target session duration if a timeout occurs.  


Next, we characterize the network congestion which will cause the timeouts.  
  Let $Y$ be the delay experience by a probing packet that traverses a link with capacity
   $C$ packets/s 
  subject to  exogenous (background) traffic with arrival rate $\Lambda$ packets/s and size exponentially distributed with mean $M$.  
  The CDF of $Y$ is given by  $F_Y(y)=P(Y < y)$.  Then, the probability that a 
  license renewal request
  succeeds is given by $q=P(Y  < \tau)$. 
  In the remainder of this paper,
   we assume that the delay is characterized by an 
   M/M/1 queue, and that the overhead caused by 
 license requests into the link is negligible compared to the exogenous traffic. 
 Then, it follows from~\cite[equation (5.119)]{kleinrock} that
 \begin{equation} 
q=1-e^{-( MC-\Lambda)\tau}
\label{MM1_waiting_time}
\end{equation}  



A timeout occurs if the target session duration is greater than the time until a renewal
request fails.  Therefore, 
the timeout probability p is given by 
  \begin{equation}
  p = P(timeout) = P(L>D)= D^{\star}(s) \Big|_{s=\mu} = D^{\star}(\mu)
  \label{P_timeout1}
  \end{equation}
 where $D^{\star}(\mu)$ is the Laplace transform of $D$  given by \eqref{D_star}, evaluated
 at the point		 $s=\mu$.
 
 Our goal is to obtain a simple expression for $p$. 
To this aim, we substitute~\eqref{MM1_waiting_time} into \eqref{D_star_fim}  and make use
of  \eqref{P_timeout1} to obtain $p$,
   \begin{eqnarray}
    p=P(timeout)&=&  e^{-\mu/r}\left( \frac{e^{-( MC-\Lambda)\tau}  }
    {1- e^{-{\mu}/{r}}\left(1- e^{-( MC-\Lambda)\tau}\right)}\right) 
  \end{eqnarray}  
  Note that if $q=0$ then $p=e^{-\mu/r}$ because the first license renewal request occurs
   $1/r$ time units after the license is obtained at the first place.  The probability that
   the license cannot be initially obtained  is captured through $P(blocking)$.
  
%    \begin{eqnarray}
%     D(z) &=&  N(z) D_i(z)\\
%     N(z) &=& \frac{F(t)z  }{1- z F(t)} \\
%     D_i(z) &=& z^{(\frac{1}{r})}\\
%     D(z) &=& z^{\frac{1}{r}}\bigg( \frac{F(t)z  }{1- z F(t)}\bigg) \\
%     z^{\frac{1}{r}}\bigg( \frac{F(t)z  }{1- z F(t)}\bigg) &\Longleftrightarrow& N(k-\frac{1}{r})\\    
%     D(k) &=& N(k-\frac{1}{r})= F(t)^{k-1-\frac{1}{r}}(1-F(t))\\
%   \end{eqnarray}
%   
  
  After some algebric manipulation, is possible to derive a explicit formula for the capacity in function of the desired timeout probability p:
  
  \begin{equation}
  C = \frac{1}{M}\bigg(\Lambda +\frac{1}{\tau}ln\bigg(\frac{p(e^{\frac{\mu}{r}}-1)}{p-1}  \bigg)\bigg)
  \label{Capacity}
  \end{equation}


\section{Multiple pools}



\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.6\textwidth, angle =270 ]{remote_pool.eps}
\end{center}
\caption{Remote License Servers}
\label{P_timeout}
\end{figure}


% \begin{equation}
% P(bloqueio)=\frac{\binom{M_1}{L}(\frac{\lambda}{\mu})^{L_1}}{\sum^{L_1}_{i=0}\binom{L_1}{i}(\frac{\lambda}{\mu})^i}+ \frac{\binom{M_2}{L}(\frac{\lambda}{\mu})^{L_2}}{\sum^{L_2}_{i=0}\binom{L_2}{i}(\frac{\lambda}{\mu})^i}
% \end{equation}


\begin{equation}
P(bloqueio)=\sum^N_{i=1}\frac{S_i}{S}\frac{\binom{S_i-1}{L}(\frac{\lambda}{\mu})^{L_i}}{\sum^{L_i}_{j=0}\binom{S_i-1}{j}(\frac{\lambda}{\mu})^j}
\end{equation}


\begin{equation}
P(timeout)=0
\end{equation}



\begin{equation}
Custo=a*L+b*C
\end{equation}

Goal: minimize costs to serve requests under availability constraints
  

\section{Private cloud remote to users}

In this scenario all servers are centralized in a private cloud located in a centralized datacenter. The question here is to evaluate the tradeoff of increasing capacity versus the economy of 
reducing both the quantity of servers and number os licenses.


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.6\textwidth, angle =270 ]{General_centralized.eps}
\end{center}
\caption{Private Cloud with Centralized Servers}
\label{P_timeout}
\end{figure}

  

\subsubsection{Immediate timeout after expiration (without resets)}

[Assume that the license is not reset after it is checked]

First, assume that $r=\infty$, and that $W$ is constant, $W=w$.  Let $X \sim \textrm{Exp}(\mu)$. Then,
\begin{equation}
P(timeout)=P(W< X)  = e^{-\mu  W}
\end{equation}
More generally, if $W$ has general distribution, with transform $W^{\star}(s)$,
\begin{equation}
P(timeout)=P(W< X)  = W^{\star}(\mu)
\end{equation}

 
\subsubsection{Non-immediate timeout after expiration (without resets)}

[Assume that the license is not reset after it is checked]


Now assume that license is checked at rate $r < \infty$, and that the mean time between 
license checks is exponentially distributed. Let $Y \sim \textrm{Exp}(r)$.   
  Let $X \sim \textrm{Exp}(\mu)$ and assume that $W$ is general with transform $W^{\star}(s)$.
\begin{eqnarray}
P(timeout) &=& P(timeout| W< X) P(W<X) \label{eq1} \\
&=&  P(X-W > Y | W <X)  W^{\star}(\mu) \label{eq2} \\
&=& P(X>Y) W^{\star}(\mu) \label{eq3} \\
&=& \frac{r}{r+\mu}  W^{\star}(\mu) 
\end{eqnarray}  
where \eqref{eq3} follows from \eqref{eq2} due to the memoryless property of the exponential distribution.
  
  
Note that 
\begin{enumerate}
\item if $W$ is a constant, we have $W^{\star}(s) = e^{-s W}$,
\begin{eqnarray}
P(timeout) &=& \frac{r}{r+\mu} e^{-\mu W}
\end{eqnarray}  
\item if $W$ is exponentially distributed with rate $1/w$, we have $W^{\star}(s) = \frac{1/w}{(1/w) + s}$,
\begin{eqnarray}
P(timeout) &=& \frac{r}{r+\mu} \frac{1/w}{(1/w) + \mu}
\end{eqnarray}  
\end{enumerate}

\subsubsection{Timeout with license resets}

(use results of queues with vacations \url{https://www.youtube.com/watch?v=ULQ646sAn9U&list=UU2zBgk83M87ZOBPZLXHhNyw})

Every time the license is checked, it is reset.  License is checked 
at rate $r < \infty$, and  the mean time between 
license checks is exponentially distributed. Let $Y \sim \textrm{Exp}(r)$.   
  Let $X \sim \textrm{Exp}(\mu)$ and assume that $W$ is the expiration time,
  since the last check, and is general with transform $W^{\star}(s)$.

  
  Let $D_i$ be the duration of the $i$-th subinterval in which the license is checked.
  Let $N$ be the number of times that the license is checked, 
  before it expires, without counting the last trial.  
   Let $D$ be the time until expiration.  
  
  \begin{eqnarray}
  D_i &=& \min(Y,W) \\
  D &=& D_0 + D_1 + D_2 + \ldots + D_N + D_{N+1} \\
  D^\star(s) &=&  N(z) \Big|_{z=F^{\star}(s)} E^{\star}(s)
  \end{eqnarray}
  where
  \begin{eqnarray}
  F &=& Y | Y < W \\
   F^\star(s) &=&  \frac{(1-W^{\star}(r+s))}{(1-W^{\star}(s))} \frac{r}{r+s} \label{eqb} \\
  D_{N+1} &=& W | W < Y \\
  E &=& D_{N+1} \\
  E^{\star}(s) &=& \frac{W^{\star}(s+r)}{W^{\star}(r)} \label{eqe} \\
  N &\sim& Geometric(W^{\star}(r)) \\
  P(N=n) &=& (1-W^{\star}(r))^{n} (W^{\star}(r))\\
  N(z) &=& \frac{W^{\star}(r)  }{1- z (1- W^{\star}(r))} 
  \end{eqnarray}
  The timeout probability is the probability that the process does not end before $D$,
  \begin{equation}
  P(timeout) = D^{\star}(\mu)
  \end{equation}
  
  
  Where \eqref{eqb} and \eqref{eqe} follow from slides 7 and 3 in \url{http://www.dcc.ufrj.br/~sadoc/ad20142/espertrans.pdf}
  
  

  
 






\begin{comment}
\section{Numerical Examples}

Fazendo-se $\mu_c=1$, $\lambda_c=1$, $M=20$, $i=2$, $M_i=10$ temos que 

\begin{equation}
\rho=\frac{\lambda_c} {\mu_c C} = \frac{1}{C}
\end{equation}



e como a aplicacao apresenta um requisito de 100 ms
 
\begin{equation}
P(timeout)=1-\bigg(1-\frac{1}{C}e^{-(C-1)0.1}\bigg)^r
\end{equation}

\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.6\textwidth]{P_timeout.jpg}
\end{center}
\caption{Probabilidade de erro por congestionamento}
\label{P_timeout}
\end{figure}


\begin{figure}[h]
\centering
   \subfigure[1 pool. \label{1 pool}]{
    \resizebox{0.45\textwidth}{!}{
            \includegraphics[width=0.41\textwidth]{P_bloqueio.jpg}
	  }
	}
  \quad
  \subfigure[2 pools. \label{2 pools}]{
    \resizebox{0.45\textwidth}{!}{
            \includegraphics[width=0.41\textwidth]{P_bloqueio_decentralizado.jpg}
	  }
	}

\caption{Probabilidade de Bloqueio}
\label{Probabilidade de Bloqueio}
\end{figure}
\end{comment}

%\begin{equation}
%P(W>0.1)=\frac{e^{-0.1C}}{C}
%\end{equation}

==> newrs.tex <==
\section{Numerical Examples}
\label{sec:exemplos}
In this section we numerically investigate 
the proposed model. \eat{ using a case study inspired by a real-world oil and gas setup. }
Our goals are to a) numerically illustrate the tradeoffs between blocking probability and timeout probability and b) indicate the applicability of the  
optimization problem proposed, quantifying the advantages and disadvantages of central and distributed pools of resources.  Our examples in  this section 
are motivated by the  previously mentioned  Oil \& Gas application. In this application, signaling servers associate one license to each  running instance of an application.  Therefore, in what follows we refer to \emph{licenses} and  \emph{application state resources} interchangeably.

%\subsection{Centralized pool of licenses, typical example}
The first analysis is a comparison between the blocking probability in the centralized and in the distributed case as shown in Figure  \ref{fig:P_bloq}(a).
In terms of blocking probability, the centralized architecture is always better. The logarithm of the blocking 
probability plotted in Figure \ref{fig:P_bloq}(b) shows that the advantage of the centralized architecture increases as the number of available licenses increases. \eat{ 
blocking probability decreases. } We refer to the reduction in blocking probability due to centralization as \emph{licensing statistical multiplexing gains}.  


\begin{figure}
\begin{center}
  \begin{tabular}{l r}
   \subfigure[Blocking Probability]{
    \resizebox{0.5\textwidth}{!}{ 
	    \includegraphics[width=0.95\textwidth]{P_bloqueio.eps}
	  }	  
	}  
  \subfigure[log(Blocking Probability)]{
    \resizebox{0.5\textwidth}{!}{ 
	  \includegraphics[width=0.95\textwidth]{log_P_bloqueio.eps}
	  }
	}  
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{Blocking probability, $\frac{1}{\mu} = 8$  hours, $S = 30$  users, $\rho=0.8$, blue=centralized, red=distributed versus number of 
available licenses}
\label{fig:P_bloq}
\vspace{-0.2in}
\end{figure}



Figure \ref{fig:P_timeout} shows the timeout probability due to congestion $p$ as a function of the link capacity $C$ for  $\tau=0.01$ and $\tau=0.05$. 
As the  capacity  $C$ increases,  $p$ decreases.  When $C = \infty$ (over-provisioning) we have $p=0$.  Figure \ref{fig:P_timeout} also shows the significant impact of the timeout detection threshold $\tau$. When $\tau=0.05$, a small increase in capacity can reduce $p$
to zero. When $\tau=0.01$ it is necessary to double the capacity to achieve the same result. In the limit when $\tau = \infty$ we note that   
$p=0$. On the other hand, when $\tau \approx 0$ it is impossible to deploy the centralized architecture. Roughly speaking, if an application developer wishes to allow the application to be used in different sites with a centralized floating 
licensing approach and the network capacity is small, the parameter $\tau$ should be relaxed.


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.45\textwidth]{P_timeout.eps}
\end{center}
\caption{Timeout probability due to congestion for different values of $\tau$. $\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, ,$\Lambda = 900$  pkt/s, 
$\frac{1}{M}=1250 $ Bytes, blue= $\tau = 0.01$ s, red=$\tau = 0.05$ s   }
\label{fig:P_timeout}
\end{figure}




Figure \ref{fig:P_timeout_X_rho} shows how the timeout probability due to congestion ($p$)  varies as a function of the the utilization factor for different workloads and link 
capacity ranges. \eat{Note that when  the traffic workload and the link capacity are scaled by a constant factor, the average delay is reduced by that factor. That is why } 
We vary the link capacity in the range of [10,25] (red line) and [1,15] (blue line) adjusting the offered workload accordingly.  Given a target value for $p$, the higher capacity network 
(red line)   can operate at a higher utilization level than the lower capacity network (blue line). \eat{  ($\Lambda=90$ packets/s)  for the same value of $p$. }
We referred to this effect as \emph{networking statistical multiplexing gain}
and one of its consequence is that is better to have one higher-speed link
instead of having n-parallel lower-speed links to carry the same amount of traffic \cite{pioro2004routing}.

\eat{
Figure \ref{fig:P_timeout_X_rho} illustrates one important design issue of networks called \textit{scaling} factor.
}

 





\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.45\textwidth]{P_timeout_X_rho.eps}
\end{center}
\caption{Timeout probability due to congestion ($p$). $\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, $\tau = 0.01$ s, $\frac{1}{M}=1250 $ Bytes. 
Red line: $\Lambda = 900$ pkt/s and $C=[10,25]$ Mbps. Blue line: $\Lambda = 90$ pkt/s and $C=[1,15]$ Mbps.   }
\label{fig:P_timeout_X_rho}
\end{figure}

\begin{comment}
Figure \ref{MM1_CDF.jpg} shows the system time distribution for different capacities but same utilization. Keeping utilization constant,
when capacity increases, the system time decreases 

\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.75\textwidth]{MM1_CDF.eps}
\end{center}
\caption{System time distribution for C=10 Mbps  and $\Lambda$ = 700 pkt/s (red line) and for C=1 Mbps  and $\Lambda$ =  70 pkt/s (green line). Both
curves has the same utilization factor ($\rho=0.7$)}
\label{MM1_CDF.jpg}
\end{figure}

Figure \ref{P_timeout_X_q} shows the timeout probability due to congestion versus session duration for multiple success probabilities q and
figure \ref{P_timeout_X_duration_C} shows the timeout probability due to congestion versus session duration for multiple capacities.


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.75\textwidth]{timeout_versus_duration.eps}
\end{center}
\caption{Timeout probability due to congestion versus session duration for multiple success probabilities q. $r = \frac{1}{120}$ s, 
$\tau = 0.01$ s. Red line: $q \ = \ 0.09$. Green line: $q \ = \ 0.9$. Blue line: $q \ = \ 0.99$. Magenta line: $q \ = \ 0.999$,  }
\label{P_timeout_X_q}
\end{figure}

\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.75\textwidth]{timeout_versus_duration_C.eps}
\end{center}
\caption{Timeout probability due to congestion versus session duration for multiple capacities. $r = \frac{1}{120}$ s, 
$\tau = 0.01$ s, $\Lambda$ =  90 pkt/s, $\frac{1}{M}=1250 $ Bytes. Red line: $C \ = \ 1$ Mbps. Green line: $C \ = \ 2$ Mbps.
Blue line: $C \ = \ 5$ Mbps. Magenta line: $C \ = \ 10$ Mbps,  }
\label{P_timeout_X_duration_C}
\end{figure}

\end{comment}


\begin{figure}[h!]
\hspace{-0.2in}
\bgroup
\setlength\tabcolsep{0pt}  \begin{tabular}{cc} \setlength\tabcolsep{0pt} 
      \includegraphics[width=0.55\textwidth]{3d1.eps} & \hspace{-0.1in}
	  \includegraphics[width=0.52\textwidth]{tradeoff_a_b.eps} \\
	  (a) $s_c$ (centralized architecture) & (b) contour plots  \\
\end{tabular}
\egroup
\caption{Graphical solution of optimization problem: (a) $s_c$ as a function of capacity and number of licenses,  (b)  contour plots of $c_c=L+2C'$ (magenta and green lines), $s_c=0.95$ (red curve) and $s_d=0.95$ (blue curve).   ${1}/{\mu} = {1}/{\lambda}= 8$  hours, $S = 30$ users, 
$\frac{1}{\mu} = 8$  hours, ${1}/{r} = 120$ s, $\tau = 0.01$ s, ${1}/{M}=1250 $ Bytes, $\Lambda=900$, $C_0=10$ Mbps}
\label{fig:Optimizations1}
\end{figure}

Figure \ref{fig:Optimizations1}(a) shows the centralized probability of success $s_c$ as a function of the  the number of available licenses and link capacity. 
The success probability approaches one  when both the 
link capacity and the number of licenses are increased.   Note that unilaterally   over-provisioning the link capacity or the number of licenses is not sufficient in order to achieve high values of $s_c$.  \eat{, unilaterally,  is no large enough being impossible to achieve a high $s_c$ 
by increasing only capacity or number of licenses. }




The optimization problem described in Section~\ref{sub:optimization} admits a graphical   solution. We start considering the centralized architecture.   Recall that $C'$ is the marginal capacity added to a link of initial capacity $C_0$ resulting in a link with  capacity $C=C'+C_0$. The centralized cost is given by $c_c = \alpha L+\beta nC'$. Varying the value of $c_c$, equation  $c_c = \alpha L + \beta n (C-C_0)$ characterizes a family of parallel lines in the $(L,C)$ plane, where $L=1, 2, \ldots$ and $C \ge C_0$.
The minimum value of $c_c$ for which the corresponding line    intersects the  curve associated to the constraint $s_c \ge P(SLA)$ corresponds to the optimal centralized solution. In the distributed architecture, let $L^{\star}$ be the minimum value of $L$ for which the constraint  $s_d \ge P(SLA)$ is satisfied.  As in the distributed architecture we assume that licenses and additional state resources are accessed locally,  $C'=0$. Therefore,   the optimal distributed solution occurs at  $(L,C)=(L^{\star}, C_0)$.      We compare the centralized and distributed solutions and select the one with minimum cost.

   

\eat{ 
Because there are two possible solutions defined by the constraints $s_c$ and
$s_d$, the first point that a line costs intersect $s_c$ or $s_d$ is the solution with minimum cost and the first 
constraint satisfied is the solution with minimum cost.  }


Figures \ref{fig:Optimizations1}(b),  \ref{fig:Optimizations2}(a) and \ref{fig:Optimizations2}(b) 
illustrate the  graphical  solution. \eat{ perspective on the solution to the  optimization problem. }
In all cases the population consists of 30 users and $C_0 = 10$ Mbps. When considering distributed solutions, the population is  split  equally between two distinct 
sites.   In 
Figure \ref{fig:Optimizations1}(b) the cost per license is twice the cost per Mbps, meaning that $cost=L+2C'$. 
The cost curve marked with ``23'' (magenta line) represents a scenario with $cost=L+2C'= 23$. The cost curve marked with ``29'' (green line) represents a scenario in which  
$cost=L+2C'= 29$. The red curve is a contour plot of the centralized architecture constraint  wherein $s_c=0.95$, and the blue curve is a contour plot of the distributed  architecture constraint  wherein $s_d=0.95$. In this example we have $P(SLA)=0.95$.
The  intersection  between a cost line and a constraint curve  
corresponding  to the smallest feasible cost  
occurs at the bottom of Figure~\ref{fig:Optimizations1}(b).  
This means that the distributed architecture is the best choice, $cost=c_d^{\star}=23$ and 23 is the minimum number of licenses that satisfies the $p(SLA)$ requirement. 
To achieve the same SLA, the cost of the centralized architecture would be 29. 
 

\eat{the magenta line given by $cost=2L+2C'=23$ and the blue line which is the constraint given by $s_d$.  At this point the cost is minimized across all feasible solutions. }


Figure \ref{fig:Optimizations2}(a) shows  the graphical solution of the optimization problem when the cost per Megabit/s is five times the cost per 
license. In this case the distributed architecture is  again the best solution.  
The intersection  between a cost line and a constraint curve  
corresponding  to the smallest feasible cost  
occurs at the bottom of Figure~\ref{fig:Optimizations2}(a), and involves the cost line  $cost=c_d^{\star}=L+10C'=22$ (magenta line) and the distributed architecture constraint given by $s_d=0.95$ (blue line).  
In this case, to achieve the same SLA the cost of the centralized architecture would be   $cost=L+10C'=98$. The communication cost makes the centralized architecture not viable.  

\eat{

the first point of intersection between a cost line and a constraint function 
is the intersection between the magenta line given by }

Figure \ref{fig:Optimizations2}(b) shows an example where the centralized architecture outperforms the distributed one.  The cost per license is five times the cost per Megabit/s. In this case, the magenta  line associated to a cost of ``212'', $cost=c_c^{\star}=10L+2C'=212$, intersects  the red curve associated to the centralized architecture constraint, $s_c=0.95$.  The blue curve corresponding  to the distributed architecture constraint  does not intersect  lines associated to costs smaller than or equal to 230. 

\eat{
The  intersection between the contour red curve representing
 an the green curve marked with 
``208'' where .
}

 \eat{ lines with costs of and a constraint curve  
corresponding  to the smallest feasible cost  
occurs at the bottom of
the centralized architecture  is the best solution.    the first
}

\begin{figure}[h!]
\begin{center}
  \begin{tabular}{l r}
     \subfigure[]{
    \resizebox{0.5\textwidth}{!}{ 
	  \includegraphics[width=0.95\textwidth]{tradeoff_10a_b.eps}
	  }
	}
   \subfigure[]{
    \resizebox{0.5\textwidth}{!}{ 
	  \includegraphics[width=0.95\textwidth]{tradeoff_a_10b.eps}
	  }
	}
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{Graphical views of optimization problem: (a)$c_c=L+10C'$,  (b)$c_c=10L+2C'$,  $\frac{1}{\mu} = \frac{1}{\lambda}= 8$  hours, S = 30 users, 
$\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, $\tau = 0.01$ s, $\frac{1}{M}=1250 $ Bytes, $\Lambda=900$, $C_0=10$ Mbps }
\label{fig:Optimizations2}
\end{figure}



\begin{comment}
\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.75\textwidth]{tradeoff_a_b.eps}
\end{center}
\caption{Graphical solution of the optimization problem. Contour plot of p(success) in centralized architecture (red line), 
distributed architecture (blue) when P(sla)=0.95 and the cost/Mbps=cost/License. $\frac{1}{\mu} = \frac{1}{\lambda}= 8$  hours, S = 30 users, 
$\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, $\tau = 0.01$ s, $\frac{1}{M}=1250 $ Bytes, $\Lambda=900$} 
\label{tradeoff_a_b}
\end{figure}


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.75\textwidth]{tradeoff_10a_b.eps}
\end{center}
\caption{Graphical solution of the optimization problem. Contour plot of p(success) in centralized architecture (red line), 
distributed architecture (blue) when P(sla)=0.95 and the cost/Mbps is ten times the cost/License. $\frac{1}{\mu} = \frac{1}{\lambda}= 8$  hours, S = 30 users, 
$\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, $\tau = 0.01$ s, $\frac{1}{M}=1250 $ Bytes, $\Lambda=900$}
\label{tradeoff_10a_b}
\end{figure}


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.75\textwidth]{tradeoff_a_10b.eps}
\end{center}
\caption{Graphical solution of the optimization problem. Contour plot of p(success) in centralized architecture (red line), 
distributed architecture (blue) when P(sla)=0.95 and the cost/license is ten times the cost/Mbps. $\frac{1}{\mu} = \frac{1}{\lambda}= 8$  hours, S = 30 users, 
$\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, $\tau = 0.01$ s, $\frac{1}{M}=1250 $ Bytes, $\Lambda=900$}
\label{tradeoff_a_10b}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}
\begin{center}
  \begin{tabular}{l r}
   \subfigure[]{
    \resizebox{0.5\textwidth}{!}{ 
	    \includegraphics[width=0.95\textwidth]{P_availability.eps}
	  }	  
	}  
  \subfigure[]{
    \resizebox{0.5\textwidth}{!}{ 
	  \includegraphics[width=0.95\textwidth]{tradeoff_a_b.eps}
	  }
	}\\ 
  \subfigure[]{
    \resizebox{0.5\textwidth}{!}{ 
	  \includegraphics[width=0.95\textwidth]{tradeoff_10a_b.eps}
	  }
	}
   \subfigure[)]{
    \resizebox{0.5\textwidth}{!}{ 
	  \includegraphics[width=0.95\textwidth]{tradeoff_a_10b.eps}
	  }
	}
\end{tabular}
\end{center}
\caption{(a) $s_c$, Graphical views of optimization problem: (b)$C=L+C$, (c)$C=L+5C$,(d)$C=5L+C$,  $\frac{1}{\mu} = \frac{1}{\lambda}= 8$  hours, S = 30 users, 
$\frac{1}{\mu} = 8$  hours, $\frac{1}{r} = 120$ s, $\tau = 0.01$ s, $\frac{1}{M}=1250 $ Bytes, $\Lambda=900$}
\label{fig:Optimizations}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[h]
\centering
   \subfigure[1 pool. \label{1 pool}]{
    \resizebox{0.45\textwidth}{!}{
            \includegraphics[width=0.41\textwidth]{P_bloqueio.jpg}
	  }
	}
  \quad
  \subfigure[2 pools. \label{2 pools}]{
    \resizebox{0.45\textwidth}{!}{
            \includegraphics[width=0.41\textwidth]{P_bloqueio_decentralizado.jpg}
	  }
	}

\caption{Probabilidade de Bloqueio}
\label{Probabilidade de Bloqueio}
\end{figure}
\end{comment}

==> questions.tex <==
\section{Some Interesting Questions}
\label{sec:question}


Key question to address: how many licenses to leave in a centralized server, and how many to distribute among
pools?

Trade-offs involved:
\begin{enumerate}
\item if licenses are centralized in a remote server, we decrease $P(blocking)$ (due to 
statistical multiplexing), but we increase $P(timeout)$ (because the networking connection is weaker). 
\item in addition, as it will take longer to run the sections when they are decentralized,
this will not only increase $P(timeout)$ but also increase $P(blocking)$  as the blocking
probability also depends on the duration of sessions
\item another interesting point is to consider users that retry to access the system after timeout.
Therefore, timeouts will also increase the effective arrival rate of request, which might further
increase blocking
\end{enumerate}


We start with only the first trade-off in bullet 1 above  and later consider  bullet 2 above as well, together with bullet 1.

 \clearpage
  \pagebreak
